Pengines: Web Logic Programming Made Easy

When developing a (web) interface for a deductive database, functionality required by the client is provided by means of HTTP handlers that wrap the logical data access predicates. These handlers are responsible for converting between client and server data representations and typically include options for paginating results. Designing the web accessible API is difficult because it is hard to predict the exact requirements of clients. Pengines changes this picture. The client provides a Prolog program that selects the required data by accessing the logical API of the server. The pengine infrastructure provides general mechanisms for converting Prolog data and handling Prolog non-determinism. The Pengines library is small (2000 lines Prolog, 150 lines JavaScript). It greatly simplifies defining an AJAX based client for a Prolog program and provides non-deterministic RPC between Prolog processes as well as interaction with Prolog engines similar to Paul Tarau's engines. Pengines are available as a standard package for SWI-Prolog 7.

==> rpc.tex <==
\section{The implementation of pengine\_rpc/3}
\label{sec:penginerpc}

The code below shows the full source code that realises
\predref{pengine\_rpc}{3}, running a Prolog code fully transparently in
another Prolog process using HTTP requests. The entry predicate creates
a result template from the variables in \arg{Query}. It uses
SWI-Prolog's \predref{setup\_call\_cleanup}{3} to destroy the remote
pengine as soon as we no longer have need for it.  The event responses
are briefly commented in the source.

\begin{verbatim}
pengine_rpc(URL, Query, QOptions) :-
    meta_options(is_meta, QOptions, Options),
    term_variables(Query, Vars),
    Template =.. [v|Vars],
    setup_call_cleanup(
        pengine_create([ server(URL), id(Id) | Options ]),
        wait_event(Query, Template, Options),
        pengine_destroy_and_wait(Id)).

pengine_destroy_and_wait(Id) :-
    pengine_destroy(Id),
    pengine_event(destroy(Id)).

wait_event(Query, Template, Options) :-
    pengine_event(Event),
    process_event(Event, Query, Template, Options).

% create --> ask query
process_event(create(ID, _), Query, Template, Options) :-
    pengine_ask(ID, Query, [template(Template)|Options]),
    wait_event(Query, Template, Options).
% remote signalled exception.  re-throw
process_event(error(_ID, Error), _Query, _Template, _Options) :-
    throw(Error).
% remote failed.  fail.
process_event(failure(_ID), _Query, _Template, _Options) :-
    fail.
% remote wants input, read and send reply
process_event(prompt(ID, Prompt), Query, Template, Options) :-
    pengine_rpc_prompt(ID, Prompt, Reply),
    pengine_send(ID, input(Reply)),
    wait_event(Query, Template, Options).
% remotes wants output, print it.
process_event(output(ID, Term), Query, Template, Options) :-
    pengine_rpc_output(ID, Term),
    pengine_pull_response(ID, Options),
    wait_event(Query, Template, Options).
% remote debug event.  Relay to local debug.
process_event(debug(ID, Message), Query, Template, Options) :-
    debug(pengine(debug), '~w', [Message]),
    pengine_pull_response(ID, Options),
    wait_event(Query, Template, Options).
% remote sends last result set.
process_event(success(_ID, Solutions, false), _Query, Template, _Options) :- !,
    member(Template, Solutions).
% remote sends result set.  There can be more
process_event(success(ID, Solutions, true), Query, Template, Options) :-
    (   member(Template, Solutions)
    ;   pengine_next(ID, Options),
        wait_event(Query, Template, Options)
    ).

is_meta(src_predicates).

% hook pengine I/O
:- multifile prompt/3, output/2.

pengine_rpc_prompt(ID, Prompt, Term) :-
    prompt(ID, Prompt, Term0), !,
    Term = Term0.
pengine_rpc_prompt(_ID, Prompt, Term) :-
    setup_call_cleanup(
        prompt(Old, Prompt),
        read(Term),
        prompt(_, Old)).

pengine_rpc_output(ID, Term) :-
    output(ID, Term), !.
pengine_rpc_output(_ID, Term) :-
    print(Term).
\end{verbatim}

